Depression detection from Social Media Bangla Text Using Recurrent Neural Networks

Emotion artificial intelligence is a field of study that focuses on figuring out how to recognize emotions, especially in the area of text mining. Today is the age of social media which has opened a door for us to share our individual expressions, emotions, and perspectives on any event. We can analyze sentiment on social media posts to detect positive, negative, or emotional behavior toward society. One of the key challenges in sentiment analysis is to identify depressed text from social media text that is a root cause of mental ill-health. Furthermore, depression leads to severe impairment in day-to-day living and is a major source of suicide incidents. In this paper, we apply natural language processing techniques on Facebook texts for conducting emotion analysis focusing on depression using multiple machine learning algorithms. Preprocessing steps like stemming, stop word removal, etc. are used to clean the collected data, and feature extraction techniques like stylometric feature, TF-IDF, word embedding, etc. are applied to the collected dataset which consists of 983 texts collected from social media posts. In the process of class prediction, LSTM, GRU, support vector machine, and Naive-Bayes classifiers have been used. We have presented the results using the primary classification metrics including F1-score, and accuracy. This work focuses on depression detection from social media posts to help psychologists to analyze sentiment from shared posts which may reduce the undesirable behaviors of depressed individuals through diagnosis and treatment.

==> Tex_Code/3.method/A.dataset.temp.tex <==
\subsection{Dataset Creation}\label{AA}
We extract facebook posts from five different facebook groups consisting of authenticated members, using Facebook Graph API version 3.0. Some annotated sample posts shown in Table II. We collect facebook posts with posts author names and separately collect the the members list using Graph API. We manually label the members as Male and Female. Then we assign the author gender by cross multiplying the posts data with author name and labeled members list.

We do not use user API to get user gender since we do not have user level permission. For labeling members we tokenize the unique member names and we manually assign the Male, Female and Common to these tokens. For example from member name "Sajid Hasan" we get tokens "Sajid" and "Hasan" to which we assign "Male" and "Common" labels. On the other hand, from member name "Sanjida Hasan" we get tokens "Sanjida" and "Hasan" to which we assign "Female" and "Common" labels. We collect 10,000 unique members name and we get 2000 Male token, 2500 Female token, 1500 common tokens. Then we get label for original members name from the assigned tokens.

==> Tex_Code/3.method/E.latex_advice.tex <==
\subsection{\LaTeX-Specific Advice}
Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

==> Tex_Code/3.method/F.mistakes.tex <==
\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.

==> Tex_Code/3.method/G.authors.tex <==
\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).

==> Tex_Code/3.method/H.headings.tex <==

\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

==> Tex_Code/3.method/I.figures.tex <==
\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and  bottom of columns. Avoid placing them in the middle of columns. Large figures and tables may span across both columns. Figure captions should be  below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation ``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.

==> Tex_Code/6.acknowledge/acknowledgement.tex <==


The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.

==> Tex_Code/7.references/nokol.tex <==

\bibitem{b1} Corney, M., Vel, O. d., Anderson, A., and Mohay, G., “Gender-preferential text mining of e-mail discourse,” in Computer Security Applications Conference(CSAC), Las Vegas, USA, Dec 9-13, 2002.

\bibitem{b2} Keselj, V., Peng, F., Cercone, N., and Thomas, C., “N-gram-based author profiles for authorship attribution,” in Pacific Association for Computational Linguistics, Halifox, Canada, Aug 22-25,2003.

\bibitem{b3} Rangel, F., Rosso, P., Potthast, M., and Stein, B., “Overview of the 5th author profiling task at pan 2017: Gender and language variety identification in twitter,” in Notebook for PAN at CLEF, Dublin, Ireland, Sept 11-14 , 2017.
\bibitem{b4} Vollenbroek, M. B. o., Carlotto, T., Kreutz, T., Medvedeva, M., Pool, C., Bjerva, J., Haagsma, H., and Nissim, M., “Content-centric age and gender profiling,” in Notebook for PAN at CLEF, Évora, Portugal, Sept 05-08 , 2016.
\bibitem{b5} Lim, W.-Y., Goh, J., and Thing, V. L. L., “Content-centric age and gender profiling,” in Notebook for PAN at CLEF, Valencia, Spain, Sept 23-26, 2013.
\bibitem{b6} Rosenthal, S., Agarwal, A., and McKeown, K., “Columbia nlp: Sentiment detection of sentences and subjective phrases in social media,” in Semantic Evaluation (SemEval), Dublin, Ireland, Aug 23-24, 2014.
\bibitem{b7} Sboev, A., Litvinova, T., Voronina, I., Gudovskikh, D., and Rybka, R., “Deep learning network models to categorize texts according to author’s gender and to identify text sentiment,” in Computational Science and Computational Intelligence (CSCI), Las Vegas, USA, Dec 15-17, 2016.
\bibitem{b8} lsmearat, K., Al-Ayyouba, M., Al-Shalabi, R., and Kanaanbt, G., “Author gender identification from arabic text,” Journal of Information Security and Applications , vol. 35, no. 8, pp. 85–95, 2017.
\bibitem{b9} Bsir,  B. and Zrigui,  M.,  “Enhancing deep learning gender identification with gated recurrent units architecture in social text,” Computación y Sistemas , vol. 22, no. 3, pp. 757–766, 2018.
\bibitem{b10} Rahman, S. M., Kabir, F. M., Kabir, F. M., and Huda, N. M., “Automatic gender identification system for bengali speech,” in Electrical Information and Communication Technologies (EICT), Khulna, Bangladesh, Dec 10-12 , 2015.
\bibitem{b11} Tripto, N. I., and Ali, M. E. “Detecting Multilabel Sentiment and Emotions from Bangla YouTube Comments,” in International Conference on Bangla Speech and Language Processing (ICBSLP), Sylhet, Bangladesh, Sept 21-22 , 2018.

==> Tex_Code/7.references/references.tex <==
\printbibliography

==> Tex_Code/resource/table/3.c.stylo.translate.tex <==

\begin{table*}[htp]
\caption{Examples of Arabic and Translated Bangla \& English Words}
\label{arabic-translated-bangla}
    \centering
    \begin{tabularx}{\textwidth}{| X | X | X |  X |  X |}
        \hline
        Economy & Policy & Social & Sport & Negative \\ 
        \hline 
\arab{﻿اموال الدوله } & \arab{إساءة استخدام القوة} & \arab{ثقافات} & \arab{﻿كره القدم} & \arab{مهجور}\\ 
{\beng রাজ্য তহবিল } 
   & {\beng ক্ষমতার অপব্যবহার} & {\beng সংস্কৃতি} & {\beng ফুটবল} & {\beng পরিত্যক্ত} \\
State funds & Abuse of power & Culture & Football & Abandoned \\ 
        \hline 
        \arab{بنك} &\arab{وزير بالوكالة } & \arab{قبيله}& \arab{رياضه} & \arab{غير طبيعي}\\
        {\beng ব্যাংক }  & {\beng  ভারপ্রাপ্ত মন্ত্রী }    & {\beng উপজাতি} & {\beng খেলা}&  অস্বাভাবিক \\
     Bank & Minister in charge & Tribe & Sport & Abnormal
        \\
        \hline
        \arab{انهيار اقتصادي} & \arab{لجنة استشارية}  & \arab{طالبات المدارس} & \arab{ملعب} & \arab{إلغاء}\\
     {\beng অর্থনৈতিক পতন} & {\beng উপদেষ্টা কমিটি} & {\beng স্কুল} &  {\beng স্টেডিয়াম }& {\beng বাতিল } \\
      Economic Fall & Advisory Committee & School & Stadium &  Cancel
     \\
        \hline
        \arab{شركات} & \arab{مداولة} & \arab{اسره}& \arab{مباريات}& \arab{مفاجئ}\\
     কোম্পানি  & {\beng পরামর্শ} & {\beng পরিবার} & {\beng গেম} & {\beng আকস্মিক} \\
    Company & Advice & Family & Game & Sudden
     \\
        \hline
    \end{tabularx}
\end{table*} 
